Consistent Accelerated Inference via Confident Adaptive Transformers

We develop a novel approach for confidently accelerating inference in the large and expensive multilayer Transformers that are now ubiquitous in natural language processing (NLP). Amortized or approximate computational methods increase efficiency, but can come with unpredictable performance costs. In this work, we present CATs -- Confident Adaptive Transformers -- in which we simultaneously increase computational efficiency, while guaranteeing a specifiable degree of consistency with the original model with high confidence. Our method trains additional prediction heads on top of intermediate layers, and dynamically decides when to stop allocating computational effort to each input using a meta consistency classifier. To calibrate our early prediction stopping rule, we formulate a unique extension of conformal prediction. We demonstrate the effectiveness of this approach on four classification and regression tasks.

==> sections/background.tex <==
\section{Background}
\label{sec:background}

We begin with a review of conformal prediction. 
%Here, and in the rest of the paper, upper-case letters ($X$) denote random variables; lower-case letters ($x$) denote scalars, and script letters ($\mathcal{X}$) denote sets, unless otherwise specified. 
%
All proofs are deferred to Appendix~\ref{app:proofs}.
%In the following sections we assume $\emph{w.l.o.g.}$ that the input is a vector $x \in \mathcal{X}$ and the output is a class label $y \in \{1. \ldots, k\}$. In general, they can be represented differently (e.g., with structure).

%TS: $\textbf{x}$ for tensors? (it sounds weird to say that the input to the model is a scalar)

\subsection{Nonconformity measures}
\label{sec:background_nonconf}
Given a new example $x$, for every candidate label $y \in \mathcal{Y}$, conformal prediction applies a simple test to either accept or reject the null hypothesis that the pairing $(x, y)$ is correct. The test statistic for this hypothesis test is a \emph{nonconformity measure}, $\mathcal{S}\left((x, y), \mathcal{D}\right)$, where $\mathcal{D}$ is a dataset of exchangeable, correctly labeled examples. Informally, a lower value of $\mathcal{S}$ reflects that point $(x, y)$ ``conforms'' to $\mathcal{D}$, whereas a higher value of $\mathcal{S}$ reflects that $(x, y)$ is atypical relative to $\mathcal{D}$. A practical choice for $\mathcal{S}$ is model-based likelihood, e.g.,  $-\log p_\theta(y | x)$, where $\theta$ is a model fit to $\mathcal{D}$ using some learning algorithm $\mathcal{A}$ (such as gradient descent).
%
It is also important that $\mathcal{S}$ preserves exchangeability of its inputs. Let $Z_j := (X_j, Y_j)$, $j = 1,\ldots, n$ be the training data. Then, for test point $x \in \mathcal{X}$ and candidate label $y \in \mathcal{Y}$,  we calculate the \emph{nonconformity scores} for $(x, y)$ as:
\begin{align}
\label{eq:nonconf}
\begin{split}
    V^{(x, y)}_j &:= \mathcal{S}(Z_j, Z_{1:n} \cup \{(x, y)\}),\\
    V^{(x, y)}_{n+1} &:= \mathcal{S}((x, y), Z_{1:n} \cup \{(x, y)\}).
\end{split}
\end{align}
Note that this formulation, referred to as \emph{full} conformal prediction, requires running the learning algorithm $\mathcal{A}$ that underlies $\mathcal{S}$ potentially many times for every new test point (i.e., $|\mathcal{Y}|$ times). ``Split'' conformal prediction~\cite{Papadopoulos08}---which uses a held-out training set to learn $\mathcal{S}$, and therefore also preserves exchangeability---is a more computationally attractive alternative, but comes at the expense of predictive efficiency when data is limited.
%As a side result, in \S\ref{sec:metalearning} we show how meta-learning $\mathcal{S}$ allows for computationally efficient full conformal prediction. 

% \begin{definition}[Nonconformity measure] Let $\mathcal{Z} := \mathcal{X} \times \mathcal{Y}$ be the space of examples $(X,Y)$, and let $\mathcal{Z}^{(*)} := \bigcup_{d \geq 1} (\mathcal{X} \times \mathcal{Y})^{d}$ be the space of datasets of examples  $\mathcal{D}$, of any size $d \geq 1$. A \emph{nonconformity measure} $\mathcal{S}$ is then a measurable mapping $\mathcal{S} \colon \mathcal{Z} \times \mathcal{Z}^{(*)} \rightarrow {\mathbb{R}}$, that assigns a real-valued score to any example $(X, Y)$, indicating how ``different'' it is from a reference dataset $\mathcal{D}$.
% %
% \end{definition}

\subsection{Conformal prediction}
\label{sec:background_cp}
To construct the final \emph{prediction} for the new test point $x$, the classifier tests the nonconformity score for each label $y$, $V_{n+1}^{(x, y)}$, against a desired significance level $\epsilon$, and includes all $y$ for which the null hypothesis---that the candidate pair $(x,y)$ is \emph{conformal}---is not rejected. This is achieved by comparing the nonconformity score of the test candidate to the scores computed over the first $n$ labeled examples.
This comparison leverages the quantile function, where for a random variable $V$ sampled from distribution $F$ we define
\begin{equation}
    \mathrm{Quantile}(\beta; F) := \inf\{v \colon F(v) \geq \beta\}.
\end{equation}
In our case, $F$ is the empirical distribution over the $n+1$ nonconformity scores. However, as we do not know the last value of $V_{n+1}^{(x, y)}$ for the true $y^*$, we use an ``inflated'' quantile:
\begin{lemma}[Inflated quantile]
\label{lemma:quantile}
Assume that $V_j$, $j=1,$ $\ldots, n+1$ are exchangeable random variables.
Then for any $\beta \in (0, 1)$,  $\mathbb{P}\left(V_{n+1} \leq \mathrm{Quantile}(\beta, V_{1:n} \cup \{\infty\})\right) \geq \beta.$
% \begin{equation}
%   \mathbb{P}\left(V_{n+1} \leq \mathrm{Quantile}(\beta, V_{1:n} \cup \{\infty\})\right) \geq \beta.  
% \end{equation}
% \begin{equation}
% \label{eq:quantile}
% \mathbb{P}\left(V_{n+1} \leq \mathrm{Quantile}(\beta, V_{1:n} \cup \{\infty\})\right) \geq \beta.
% \end{equation}
\end{lemma}

Conformal prediction then guarantees marginal coverage by including all labels $y$ for which $V_{n+1}^{(x, y)}$ is below the inflated empirical quantile of the $n$ training points, as summarized:

\begin{theorem}[CP, \citet{vovk2005algorithmic}]
\label{thm:conformalprediction}
Assume that examples $(X_j, Y_j)$, $j=1,\ldots, n+1$ are exchangeable. For any nonconformity measure $\mathcal{S}$ and $\epsilon \in (0, 1)$, define the conformal set (based on the first $n$ examples) at  $x \in \mathcal{X}$ as
\begin{equation*}
\label{eq:csetconstruction}
\resizebox{1\hsize}{!}{$\displaystyle
	\cset(x) := \Big \{ y \in \mathcal{Y} \colon 
    V_{n+1}^{(x,y)} \leq \mathrm{Quantile}(1 - \epsilon;\, V_{1:n}^{(x, y)} \cup \{\infty\}) \Big\}.
$}
\end{equation*}
Then $\cset(X_{n+1})$ satisfies Eq.~\eqref{eq:marginalcoverage}.
\end{theorem}
